Learning to Predict 3D Objects with an Interpolation-based Differentiable Renderer

Many machine learning models operate on images, but ignore the fact that images are 2D projections formed by 3D geometry interacting with light, in a process called rendering. Enabling ML models to understand image formation might be key for generalization. However, due to an essential rasterization step involving discrete assignment operations, rendering pipelines are non-differentiable and thus largely inaccessible to gradient-based ML techniques. In this paper, we present {\emph DIB-R}, a differentiable rendering framework which allows gradients to be analytically computed for all pixels in an image. Key to our approach is to view foreground rasterization as a weighted interpolation of local properties and background rasterization as a distance-based aggregation of global geometry. Our approach allows for accurate optimization over vertex positions, colors, normals, light directions and texture coordinates through a variety of lighting models. We showcase our approach in two ML applications: single-image 3D object prediction, and 3D textured object generation, both trained using exclusively using 2D supervision. Our project website is: https://nv-tlabs.github.io/DIB-R/

==> doc/3_diffshader.tex <==

\vspace{-5pt}
\section{{\model }: Interpolation-based Differentiable Renderer}
\vspace{-5pt}
In this section, we introduce our {\model }. Treating rasterization as an interpolation of vertex attributes allows realistic images to be produced, whose gradients can be fully back-propagated through all predicted vertex \vertexdatas. 

% First, discuss render pipeline in OpenGL
\vspace{-7pt}
\subsection{Rendering Pipeline}
\vspace{-5pt}
Many popular rendering APIs, such as OpenGL~\cite{woo1999opengl} and DirectX3D~\cite{luna2012introduction}, decompose the process of rendering 3D scenes into a set of sequential user-defined programs, referred to as \emph{shaders}. While there exist many different shader types, the vertex, rasterization, and fragment shaders the three most important steps for establishing a complete rendering pipeline. When rendering an image from a 3D polygon mesh, first, the vertex shader projects each 3D vertex in the scene onto the defined 2D image plane. Rasterization is then used to determine which pixels are covered and in what manner, by the primitives these vertices define. Finally, the fragment shader computes how each pixel is colored by the primitives which cover it.  

%While each of these shaders is essential for any colored rendering, for the purposes of designing a differentiable rending pipeline, rasterization must take the highest consideration due to the inherently non-differentiable operations which it requires. In contrast, 
The vertex and fragment shaders can easily be defined such that they are entirely differentiable. By projecting 3D points onto the 2D image plane by multiplying with the corresponding 3D model, view and projection matrices, the vertex shader operation is directly differentiable. In the fragment shader, pixel colors are decided by a combination of local properties including assigned vertex colors, textures, material properties, and lighting. While the processes through which this information are combined can vary with respect to the chosen rendering model, in most cases this can be accomplished through the application of fully differentiable arithmetic operations. All that remains for our rendering pipeline is the rasterization shader which presents the main challenge due to the inherently non-differentiable operations which it requires. In the following section we describe our method for rasterizing scenes such that the derivatives of this operation can be analytically determined. % We note that our approach in its current form does not support handling occlusion. While pixels could be covered by multiple faces with different depth, our approach only considers the most front face and is thus limited in the scenes it can handle. Accounting for occlusion is future work. % \alec{This is not clear enough. Is occlusion handled per-iteration via rasterization and keeping only the closest fragment (z-buffer) as Paparazzi does? Or is every triangle that lands on a pixel considered to be rendered? If it's the later is the color taken as an average?} \wz{the former}
% \alec{Still not clear. This seems to contradict Eq. 6} \wz{put the explanation at the end}

\vspace{-6pt}
\subsection{Differentiable Rasterization}
\vspace{-5pt}

\iffalse
\begin{table}[t!]
	% \begin{minipage}{0.2\textwidth}
    % \includegraphics[width=1.0\textwidth]{figures/fig1_points}
	% \end{minipage}
	% \begin{minipage}{0.79\textwidth}
	\begin{adjustbox}{width=\textwidth}
	\begin{tabular}{c|c|c|c|c}
		\hline
        \textbf{Vextex Data} &\textbf{ Vextex Shader} & \textbf{Rasterization} & \textbf{Fragment Data} & \textbf{Fragment Shader} \\
        \hline
        Vertices        &               &               &               &              \\
        Vertex Colors  &  Model Matrix &                   & Pixel Colors &  Color Model \\
        Tex Coords     &   View Matrix    &  Differentiable-  &Pixel Tex Coords & Texture Model \\
        Vertex Normals  & Projection Matrix  &   Rasterizer    &Pixel Normals      & Lambertian Model \\
         Light Directions  &                &                       &Pixel Light Directions      & Spherical harmonic Model \\
          Eye Directions     &                   &                       &Pixel Eye Directions      & Phong Model \\
		\hline
	\end{tabular}
	\end{adjustbox}
	% \end{minipage}
	\caption{\footnotesize Left: Differentiable Shader. For inside pixels $I_i$, we treat it as an interpolation of three points $p_0$, $p_1$ and $p_2$. For outside pixels $I_j$, we organize it as an probability map. Right: Differentiable data and shaders. With our method, we can differentiate every element(Column 1 \& 4, Vertex and Fragment Data) and apply it into every rendering model (Column 5, Frgment Shader Model). }
 	\label{tb:oglmodel}
\end{table}
\fi

\begin{table}[t!]
\vspace{-3mm}
    \centering
    \begin{minipage}{0.73\linewidth}
    \begin{adjustbox}{width=0.98\textwidth}
	\begin{tabular}{c|c|c|c|c|c|c}
		%\toprule
		\hline
        \textbf{Model} &
        \textbf{ Vertex Position} &
        \textbf{Vertex Color} &
        \textbf{Texture} &
        \textbf{Lighting} &
        \textbf{Analytic Grad.} &
        \textbf{Text. Coord.}%&
      %  \textbf{Unbiased} 
      \\
        %\midrule
        \hline
        
        OpenDR~\cite{loper2014opendr} &
        \checkmark  & \checkmark & \checkmark &  \checkmark & &%& \checkmark
        \\
               N3MR~\cite{NMR} & 
        \checkmark &  & \checkmark &  \checkmark & &%& \checkmark
        \\
                        % MC Render~\ci
                        Paparazze~\cite{paparazzi} &
        \checkmark &  &  & \checkmark & \checkmark &%& \checkmark 
        \\
        SoftRas-Mesh~\cite{liu2019soft} & 
        \checkmark & & & &  \checkmark &%& \checkmark 
        \\
        
        SoftRas-Colour~\cite{liu2019soft_v2} & 
        \checkmark & \checkmark & & &  \checkmark &%& \checkmark 
        \\
        U3MM~\cite{genova2018unsupervised} &
        \checkmark & \checkmark & & \checkmark & \checkmark &%& \checkmark 
        \\
        Advgeo~\cite{liuadvgeo2018} &
        \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &%& \checkmark 
        \\
        
        % MCMC \cite{} &\checkmark & \checkmark&\checkmark &\checkmark & \checkmark & \checkmark & \checkmark \\
        Ours &\checkmark & \checkmark&\checkmark &\checkmark & \checkmark & \checkmark         \\
		%\bottomrule
		\hline
	\end{tabular}
	\end{adjustbox}
	\end{minipage}
	\hspace{3mm}
	\begin{minipage}{0.22\linewidth}
	\caption{\footnotesize A comparison of different differentiable rasterization-based rendering models. %\wz{Unbiased option is used to say some dl based renderers, where the input is a mesh and output is the corresponding images, will be biased. But if we just compare with rasterization-based rendering models, I think it is fine to remove it.}
	%\alec{This is very useful. Must be careful that authors of these papers would agree with the check marks   } \wz{add neural net work based rendering, set them as biased renderer, consider put it in sup?} \alec{Try to sort the rows and columns so that the feature chart is lower triangular or at least so that missing entries are near the diagonal.} \wz{seems impossible to make it lower triangle :(}
	}
		\label{tbl:diff-dr}
		\end{minipage}
	\vspace{-5mm}
\end{table}

\begin{wrapfigure}{R}{0.25\textwidth} 
\centering
\vspace{-14pt}
\includegraphics[width=0.25\textwidth]{figures/demo.pdf}
% \includegraphics[width=0.29\textwidth]{figures/fig1_refine.pdf}
 \vspace{-15pt}
 \label{fig:demonstrate}
 \caption{\footnotesize Illustration of our Differentiable Rasterization.}
\end{wrapfigure}
% show rasterization is differentiable
% need to revise veriable names in this section and reconsider interpolation formula
In contrast to standard rendering, where a pixel's value is assigned from the closest face that covers the pixel, we treat rasterization as an interpolation of vertex \vertexdatas. Consider first only the \textbf{foreground pixels} that are covered by one or more faces. For every such pixel we perform a z-buffering test~\cite{greene1993hierarchical}, and assign it to the closest covering face. Each pixel is influenced exclusively by this face. Shown in Fig.~1, a pixel at position $\vec{p}_i$ is covered by face $f_j$ with three vertices $\vec{v}_{0}$, $\vec{v}_{1}$, $\vec{v}_{2}$, and each vertex has its own \vertexdatas: $u_{0}$, $u_{1}$, $u_{2}$, respectively. $\vec{p}_i$ and  $\vec{v}_i$ are 2D coordinates on the image plane while $u_i$ are  scalars. We compute the value of this pixel, $I_i$, using barycentric interpolation % \alec{this citation doesn't make sense and is unnecessary}~\cite{berrut2004barycentric} 
of the face's vertex \vertexdatas:
\begin{equation}
    I_i = w_0 u_{0} + w_1 u_{1} + w_2 u_{2}, 
\label{equation:interpolation}
\end{equation}
where weights $w_0$, $w_1$ and $w_2$ are calculated over the vertex and pixel positions using a differentiable functions $\Omega_k$ (provided in Appendix):\\[-2mm] 
\begin{equation}
    w_k = \Omega_k(\vec{v}_{0}, \vec{v}_{1},\vec{v}_{2}, \vec{p}_i), \quad k=0, 1, 2.
\label{equation:wfunc}
\end{equation}
With this approach, it is easy to back-propagate gradients from a loss function $L$, defined on the output image, through pixel value $I_i$ to vertex \vertexdatas {} $u_{k}$ via the chain rule:\\[-2mm]
\begin{equation}
  \frac{\partial I_i}{\partial u_k} = w_k, \quad
  \frac{\partial I_i}{\partial \vec{v}_{k}} = \sum_{m=0}^{2} \frac{\partial I_i}{\partial w_m} \frac{\partial \Omega_m}{\partial \vec{v}_{k}},
\label{equation:diff2}
\end{equation}
\begin{equation}
  \frac{\partial L}{\partial u_k} = \sum_{i=1}^N \frac{\partial L}{\partial I_i} \frac{\partial I_i}{\partial u_k}
  ,\quad 
  \frac{\partial L}{\partial \vec{v}_k} = \sum_{i=1}^N \frac{\partial L}{\partial I_i} \frac{\partial I_i}{\partial \vec{v}_k},
\label{equation:diff3}
\end{equation}
% we need to mention the 
where $N$ is the number of pixels covered by that face. Now consider pixels which no faces cover, which we refer to as \textbf{background pixels}. Notice that in the formulation above, the gradients from background pixels cannot back-propagate to any mesh \vertexdatas. However, the background pixels provide a strong constraint on the 3D shape, and thus the gradient from them provide a useful signal when learning geometry.
Take, for example, the pixel $p_{i'}$ at position $\vec{p}_{i'}$ which lies outside of face $f_j$, in Fig~1. 
%Even though the face does not directly contribute to the pixel's value currently, it has some probability to influence it after some update, and this probability is heavily related to the distance separating them.\alec{This doesn't yet make sense. There's no notion of ``probability'' unless we treat the mesh as uncertain or coming from a random distribution}
We want this pixel, despite falling slightly outside a face, to still provide a useful learning signal.
%To allow this potential influence to propagate to the learning signal, we render our images in RGBA colour space, and view the predicted alpha channel as probability of influence from all faces for every pixel. 
Inspired by~\cite{liu2019soft}, we define distance-related probability $A^j_{i'}$, that softly assigns face $f_j$ to pixel $p_{i'}$ as:
%the probability that face $f_j$ influences pixel $p_i$, as: 
\begin{eqnarray}
	{A^j_{i'}} = \exp(-\frac{d({p_{i'}}, f_j)}{\delta}),
	\label{equation:diff4}
\end{eqnarray}
where $d({p_{i'}}, f_j)$ is the distance function from pixel $p_{i'}$ to face $f_j$ in the projected 2D space, and $\delta$ is a hyper-parameter that controls the smoothness of the probability (details provided in Appendix). We then combine the probabilistic influence of all faces on a particular pixel in the following way: \\[-5mm]
\begin{eqnarray}
	{A_{i'}} = 1 - \prod_{j=1}^n (1-{A^j_{i'}}).
	\label{equation:diff5}
\end{eqnarray}
where $n$ is the number of all the faces. The combination of all $A_{i'}$ into their respective pixel positions makes up our alpha channel prediction. With definition, any background pixel can pass its gradients back to positions of all the faces with influence proportional to the distance between them in alpha channel.
%
% \alec{This is confusing. Which is used? This or the z-buffer?}\wz{we spit pixels into foreground pixels and back ground pixels, where foreground pixels we calculate gradients based on the z-buffer(each pixel is just related to one most front face that cover it). For background pixels they will be influenced by all the faces, and thus we use the formula rather than z-buffer.}
%
As all foreground pixels have a minimum distance to some face of $0$, they must receive an alpha value of 1, and so gradients will only be passed back through the colour channels as defined above.

In summary, foreground pixels, which are covered by a specific face, back-propagate gradients though interpolation while background pixels, which are not covered by any face, softly back propagate gradients to all the faces based on distance. In this way, we can analytically determine the gradients for all aspects of our rasterization process and have achieved a fully differentiable rendering pipeline. 

We note that our approach in its current form does not explicitly handle occlusion. Even though foreground pixels could be covered by multiple faces with different depth, due to z-buffering they are only influenced by the closest faces. In contrast, background pixels are related to all faces(Eq. ~\ref{equation:diff5}), however, due to distance attenuation they mostly affect faces near the outer boundary. Accounting for occlusion in an explicit way is future work. 

% For a more detailed derivation please refer to the supplementary.

% We believe our propability is a better simulation of silhouette than \cite{}. We show the difference of our propobability map and propobabilitu map in \cite{}. \cite{} use $Sigmoid$ function, which leads dard lines in face edge area. Instead, we simply use exp function and only process pixels outside faces, makes our propobability more xx adnxx.
\vspace{-5pt}
\subsection{Rendering Models}
\vspace{-5pt}
\label{subsec:rendermodels}
% The key advantage of our differentiable rasterization technique it that it can be embedded into a variety of advanced rendering models. In the following section we outline the vertex \vertexdatas the rasterizer can interpolate over and then back-propagate through, and the lighting models which the support of these \vertexdatas allows. A complete overview of this information is shown in Table ~\ref{tb:oglmodel}.

In Equation~\ref{equation:interpolation}, we define pixel values $I_i$ by the interpolation of abstract vertex {\vertexdatas} $u_0$, $u_1$ and $u_2$. As our renderer expects a mesh input, vertex positions is naturally one such \vertexdata, but we also simultaneously support a large array of other vertex {\vertexdatas } as shown in the Appendix. %Table~\ref{tb:oglmodel}, Column 1. 
In the following section we outline the vertex {\vertexdatas } the rasterization can interpolate over and then back-propagate through, and the rendering models which the support of these {\vertexdatas } allows. A complete overview of this information is shown in Appendix. %Table ~\ref{tb:oglmodel}.

\vspace{-5pt}
\subsubsection{Basic Models}
\vspace{-5pt}
Our \model {} supports basic rendering models where we draw the image directly with either vertex colors or texture. To define the basic colours of the mesh we support vertex {\vertexdatas} as either vertex colour or u,v coordinates over a learned or predefined texture map. Pixel values are determined through bi-linear interpolation of the vertex colours, or projected texture coordinates, respectively.
%or can be enhanced with the advanced lighting systems described in the next sub-section. 
%To enable these lighting effects
%we can interpolate over further mesh properties such as vertex normals and lighting direction  and learn extrinsic scene parameters such as camera position, and camera orientation. 
% We can further interpolate over more rendering properties such as vertex normals  and learn extrinsic scene parameters such as camera position, and camera orientation.  
\vspace{-5pt}
\subsubsection{Lighting Models}
\vspace{-5pt}
We also support 3 different local illumination models: Phong~\cite{Phong1975}, Lambertian~\cite{lambert1760photometria} and Spherical Harmonics~\cite{spheircalharmonic}, where the lighting effect is related to normal, light and eye directions.

To unify all the different lighting models, we decompose image color, $I$, into a combination of mesh color $I_c$ and lighting factor $I_l$ and  $I_s$: 
\begin{equation}
I = I_l I_c + I_s. 
\end{equation}
$I_c$ denotes the interpolated vertex colour or texture map values extracted directly from the vertex \vertexdatas {} without any lighting effect, $I_l$ and $I_s$ donate the lighting factors decided by specific lighting model chosen, where $I_l$ will be merged with mesh colour and $I_s$ is additional lighting effect that does not rely on $I_c$. %such as the secular effects required in the Phong Model~\cite{}. 
We first interpolate light-related {\vertexdatas} such as normals, light or eye directions in rasterization, then apply different lighting models in our fragment shader.

\textbf{Phong and Lambertian Models:}
In the Phong Model, image colour $I$ is decided by vertex normals, light directions, eye directions and material properties through the following equations: 
\begin{equation}
I_l = k_d (\vec{L} \cdot \vec{N}), \quad   \quad I_s = k_s (\vec{R} \cdot \vec{V})^{\alpha},
\end{equation}
where, $k_d$, $k_s$ and $\alpha$ are: diffuse reflection, specular reflection, and shininess constants. $\vec{L}$, $\vec{N}$, $\vec{R}$ and $\vec{V}$ are directions of light, normal, eye and reflectance, respectively, which are all interpolated vertex \vertexdatas. This results in the following definition for image colour under the Phong model:
\begin{equation}
I_{Phong} = I_c k_d (\vec{L} \cdot \vec{N})  + k_s (\vec{R} \cdot \vec{V})^{\alpha} . 
\end{equation}
As a slight simplification of full Phong shading we do not adopt ambient light and set light colour at a constant value of $1$. The Lambertian model can be viewed as a further simplification of the Phong Model, where we only consider diffuse reflection, and set $I_s$ as zero: 
\begin{equation}
I_{Lambertian} = I_c k_d (\vec{L} \cdot \vec{N}). 
\end{equation}

\textbf{Spherical Harmonic Model:}
Here,   $I_l$ is determined by normals while $I_s$ is set to $0$: 
\begin{equation}
I_{Spherical Harmonic} = I_c  \sum_{l=0}^{n-1}\sum_{m=-l}^{l}w_l^m Y_l^m(\vec{N}).
\end{equation}
where $Y_m^l$ is an orthonormal basis for spherical functions analogous to a Fourier series where $l$ is the frequency and 
% denoted with the subscript with l as the frequency and that there are 2l + 1 functions per frequency, denoted by superscripts m
% between −l to l inclusively
$w_l^m$ is the corresponding coefficient for the specific basis. To be specific, we set $l$ as 3 and thus predict 9 coefficients in total. By adjusting different $w_l^m$, different lighting effects are simulated. For more details please refer to \cite{spheircalharmonic}, Section ~2.


